The Psychological Gains from COVID-19 Vaccination: Who Benefits the Most?

We quantify the impact of COVID-19 vaccination on psychological well-being using information from a large-scale panel survey representative of the UK population. Exploiting exogenous variation in the timing of vaccinations, we find that vaccination increases psychological well-being (GHQ-12) by 0.12 standard deviation, compensating for around one-half of the overall decrease caused by the pandemic. This effect persists for at least two months, and it is associated with a decrease in the perceived likelihood of contracting COVID-19 and higher engagement in social activities. The improvement is 1.5 times larger for mentally distressed individuals, supporting the prioritization of this group in vaccination roll-outs.

==> tables/robust2-distress.tex <==
\begin{tabular}{l*{8}{c}} \hline\hline
& Main & Shocks & Local cases &  5-years & All sample & Balanced & No weights \\ \addlinespace \hline \addlinespace
1st vaccination&   -0.043** &   -0.042** &   -0.042*  &   -0.037   &   -0.031*  &   -0.024   &   -0.022*  \\
               &  (0.021)   &  (0.021)   &  (0.022)   &  (0.037)   &  (0.016)   &  (0.021)   &  (0.012)   \\
COVID-19 cases &            &            &    0.004   &            &            &            &            \\
               &            &            &  (0.003)   &            &            &            &            \\

First stage F  &  5482.95   &  5510.51   &  5497.68   &  4355.92   &  6805.95   &  4042.27   & 12553.94   \\
N              &   47,376   &   47,374   &   47,172   &   27,676   &   66,560   &   36,530   &   54,899   \\
\hline \addlinespace Sample & 40-80 & 40-80 & 40-80 & 45-55, 65-75 & all & 40-80 & 40-80  \\ \hline \hline \end{tabular}

